See, Hear, Read: Leveraging Multimodality with Guided Attention for Abstractive Text Summarization

In recent years, abstractive text summarization with multimodal inputs has started drawing attention due to its ability to accumulate information from different source modalities and generate a fluent textual summary. However, existing methods use short videos as the visual modality and short summary as the ground-truth, therefore, perform poorly on lengthy videos and long ground-truth summary. Additionally, there exists no benchmark dataset to generalize this task on videos of varying lengths. In this paper, we introduce AVIATE, the first large-scale dataset for abstractive text summarization with videos of diverse duration, compiled from presentations in well-known academic conferences like NDSS, ICML, NeurIPS, etc. We use the abstract of corresponding research papers as the reference summaries, which ensure adequate quality and uniformity of the ground-truth. We then propose FLORAL, a factorized multi-modal Transformer based decoder-only language model, which inherently captures the intra-modal and inter-modal dynamics within various input modalities for the text summarization task. FLORAL utilizes an increasing number of self-attentions to capture multimodality and performs significantly better than traditional encoder-decoder based networks. Extensive experiments illustrate that FLORAL achieves significant improvement over the baselines in both qualitative and quantitative evaluations on the existing How2 dataset for short videos and newly introduced AVIATE dataset for videos with diverse duration, beating the best baseline on the two datasets by $1.39$ and $2.74$ ROUGE-L points respectively.

==> table_figures/figure_dataset.tex <==
\begin{figure*}[!t]
  \centering
  \subfigure[Duration statistics across the dataset.]{\includegraphics[scale=0.39]{table_figures/aviate_1.png}}\hspace{1.8em}
  \subfigure[Source statistics across the dataset.]{\includegraphics[scale=0.33]{table_figures/dataset_source.png}}
  \vspace{-3mm}
  \caption{Duration and source statistics of AVIATE.}
  \label{figure:dataset}
  \vspace{-2mm}
\end{figure*}





==> table_figures/table_all_table.tex <==
% no arguments
\begin{table}[!t]
\centering
\small
\setlength{\extrarowheight}{0.8pt}

% \resizebox{0.9999\columnwidth}{!}{
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{p{2cm}|p{2.8cm}|p{2.9cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}}

& \centering \multirow{2}{*}{\bf Model} & \centering \multirow{2}{*}{\bf Modality} & \multicolumn{3}{c}{\bf AVIATE Dataset} \\\cline{4-6}


& & & \bf R-1 & \bf  R-2 & \bf R-L\\
\hline

\multirow{6}{2cm}{Extractive {\tt (Text} only)} & \multirow{2}{1.8cm}{KLSumm} & {\tt ASR} & 22.19 & 2.05 & 15.59\\
& & {\tt ASR}+{\tt OCR} & 24.27 & 2.31 & 16.92 \\ \cline{2-6}

& \multirow{2}{1.8cm}{TextRank} & {\tt ASR} & 22.15 & 2.71 & 16.42\\
& & {\tt ASR}+{\tt OCR} & 24.55 & 2.72 & 22.1  \\ \cline{2-6}

& \multirow{2}{1.8cm}{LexRank} & {\tt ASR} & 22.63 & 2.49 & 15.68\\
& & {\tt ASR}+{\tt OCR} & 24.55 & 2.72 & 22.1 \\
\hline

\multirow{8}{2cm}{Abstractive {\tt (Text} only)} & \multirow{2}{1.8cm}{PG} & {\tt ASR} & 26.27 & 2.01 & 22.96\\
& & {\tt ASR}+{\tt OCR} & 27.77 & 2.05 & 23.81  \\ \cline{2-6}

& \multirow{2}{1.8cm}{PG-MMR} & {\tt ASR} & 27.34 & 2.72 & 22.63\\
& & {\tt ASR}+{\tt OCR} & 27.82 & 3.97 & 23.93 \\ \cline{2-6}

& \multirow{2}{1.8cm}{Hi-MAP} & {\tt ASR} & 27.62 & 3.16 & 22.1\\
& & {\tt ASR}+{\tt OCR} & 28.13 & 3.87 & 22.5\\ \cline{2-6}

& \multirow{2}{1.8cm}{CopyTransformer} & {\tt ASR} & 29.93 & 3.73 & 25.13\\
& & {\tt ASR}+{\tt OCR} & 30.27 & 3.94 & 27.06\\

\hline
\hline 

\multirow{10}{2cm}{Multimodal  {\tt (Text} + {\tt Audio} + {\tt Video)}} & \multirow{2}{2.8cm}{Multimodal HA} & {\tt ASR}+{\tt A}+{\tt V} & 27.51 & 4.83 & 25.32 \\
& & {\tt (ASR}+{\tt OCR)}+{\tt A}+{\tt V} & 28.14 & 4.91 & 26.12 \\ \cline{2-6}

& \multirow{2}{2.8cm}{MulT Encoder-Decoder} & {\tt ASR}+{\tt A}+{\tt V} & 29.65 & 4.12 & 26.47 \\
& & {\tt (ASR}+{\tt OCR)}+{\tt A}+{\tt V} & 30.89 & 4.34 & 27.2 \\ \cline{2-6}

& \multirow{2}{2.8cm}{FMT Encoder-Decoder} & {\tt ASR}+{\tt A}+{\tt V} & 31.8 & 4.49 & 26.1 \\
& & {\tt (ASR}+{\tt OCR)}+{\tt A}+{\tt V} & 32.85 & 4.6 & 27.65 \\ \cline{2-6}

& \multirow{2}{2.8cm}{{MulT LM}} & {{\tt ASR}+{\tt A}+{\tt V}} & {31.71} & {4.07} & {27.58} \\
& & {{\tt (ASR}+{\tt OCR)}+{\tt A}+{\tt V}} & {33.47} & {4.12} & {28.73}
 \\ \cline{2-6}

& \multirow{2}{2.8cm}{\name} & {\tt ASR}+{\tt A}+{\tt V} & 33.26 & 6.38 & 28.52 \\
& & {\tt (ASR}+{\tt OCR)}+{\tt A}+{\tt V} & {\bf 37.13} & {\bf 11.04} & {\bf 31.47} \\

\hline

\end{tabular}}
% }
% \vspace{0.1cm}
\caption{Ablation results after incorporating  OCR generated text into the ASR generated text transcript using guided-attention for different extractive and abstractive unimodal and multimodal text summarization systems on AVIATE.}
\label{tab:ocr}
%\vspace{-10mm}
\end{table}

\newcommand{\secondtable}{% no arguments
\begin{table*}[hbtp]
\centering % centering table

\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{p{3.9cm}|p{3.6cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}}
% \hline
\multirow{2}{*}{\bf Modality} & \multirow{2}{*}{\bf Model} & \multicolumn{3}{c|}{\bf How2 } & \multicolumn{3}{c}{\bf AVIATE } \\\cline{3-8}

& & \bf R-1 & \bf  R-2 & \bf R-L & \bf  R-1 & \bf R-2 & \bf  R-L\\ 

\hline
\hline

\multirow{4}{3cm}{Extractive Systems {\tt (Text} only)} & Lead3 & 43.97 & 10.31 & 35.76 & 19.23 & 1.82 & 14.69 \\
& KLSumm & 28.64 &	\centering 12.3	& 16.2 & 24.27 & 2.31 & 16.92 \\
& TextRank & 27.48 & 12.41 & 16.55 & 22.15 & 2.71 & 16.42 \\
& LexRank & 27.95 & 12.48 & 16.98 & 22.63 & 2.49 & 15.68 \\

\hline

\multirow{5}{3cm}{Abstractive Systems {\tt (Text} only)} & Seq2Seq  & 55.32 & 23.06 & 53.9 & 26.62 & 2.88 & 23.32 \\
& PG & 51.67 & 22.65 & 50.21 & 27.77 & 2.05 & 23.81 \\
& PG-MMR & 52.9 & 23.21 & 50.24 & 27.34 & 2.72 & 22.63 \\
& Hi-MAP & 49.2 & 21.36 & 47.36 & 28.13 & 3.87 & 22.5\\
& CopyTransformer & 53.7 & 23.87 & 48.04 & 30.27 & 3.94 & 27.06 \\
\hline


\multirow{2}{3.2cm}{{\tt Video} only} & Action Ft. only & 45.21 & 12.74 & 38.5 & 22.87 & 2.78 & 17.13 \\
& Action Ft. + RNN & 48.23 & 19.1 & 46.3 & 23.54 & 2.92 & 18.21 \\

\hline
\hline

\multirow{5}{3.5cm}{Multimodel Systems {\tt (Video}+{\tt Audio}+{\tt Text)}} & Multimodal HA & 55.87 & 26.32 & 54.9 & 28.14 & 4.91 & 26.12 \\
& MulT En-De & 55.89 & 26.79 & 55.1 & 30.89 & 4.34 & 27.2 \\
& FMT En-De & 55.98 & 26.83 & 55.4 & 32.85 & 4.6 & 27.65 \\
& MulT LM & 56.13 & 26.89 & 55.41 & 33.47 & 4.12 & 28.73 \\
& \textbf{\name} & \bf 56.89 & \bf 26.93 & \bf 56.80 & \bf 37.13 & \bf 11.04 & \bf 31.47 \\

\hline

\end{tabular}}
%\vspace{0.1cm}
\caption{\name\ achieves highest performance in ROUGE-1, ROUGE-2 and ROUGE-L over text based extractive system (Lead3, KLSumm, TextRank and LexRank) and abstractive systems (Seq2Seq, PG, PG-MMR, Hi-MAP and CopyTransformer) and multimodel baselines (Multimodel HA, MulT based encoder decoder, FMT based encoder decoder, MulT based language model and \name) in How2 and AVIATE datasets.}
\label{tab:compariosn}
%\vspace{-6mm}
\end{table*}}

\newcommand{\thirdtable}{% no arguments

\begin{table*}[hbtp]

\centering % centering table

\resizebox{1\textwidth}{!}
{
\begin{tabular}{p{4.2cm}|p{2.2cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}|P{0.9cm}| P{0.9cm}|P{0.9cm}}
% \hline
\multirow{2}{*}{\bf Modality} & \multirow{2}{*}{\bf Model} & \multicolumn{4}{c|}{\bf How2 } & \multicolumn{4}{c}{\bf AVIATE } \\\cline{3-10}

& & \bf INF & \bf  REL & \bf COH & \bf FLU & \bf INF & \bf  REL & \bf COH & \bf FLU \\ 

\hline
\hline

\multirow{2}{3.5cm}{Extractive Systems {\tt \footnotesize{(Text only)}}} & KLSumm & 2.82 & 2.54 & 2.98 & 3.14 & 1.91 & 1.56 & 2.14 & 2.13  \\
& TextRank & 2.92 & 2.73 & 2.82 & 3.12 & 2.1 & 1.83 & 2.13 & 2.12   \\

\hline

\multirow{2}{3.5cm}{Abstractive Systems \footnotesize{(Text only)}} &  PG & 3.45 & 3.17 & 3.12 & 3.32 & 3.49 & 3.38 & 3.41 & \bf 3.62 \\
& CopyTrans. & 3.46 & 3.18 & 3.18 & 3.36 & 3.54 & 3.39 & 3.48 & 3.56 \\
\hline


\multirow{1}{3.5cm}{{Abstractive Systems \footnotesize{(Video only)}}}  & Action Ft.+RNN & \multirow{2}{*}{3.54} & \multirow{2}{*}{3.20} & \multirow{2}{*}{3.21} & \multirow{2}{*}{3.40} & \multirow{2}{*}{3.52} & \multirow{2}{*}{3.27} & \multirow{2}{*}{3.31} & \multirow{2}{*}{3.41} \\

\hline
\hline

\multirow{3}{3.5cm}{Multimodel Systems \footnotesize{(Video+Audio+Text)}} & FMT En-De & 3.61 & \bf 3.39 & 3.37 & 3.67 & 3.64 & 3.32 & 3.37 & 3.49  \\
& MulT LM & 3.57 &  3.38 & 3.34 & 3.68 & 3.67 & 3.39 & 3.38 & 3.45 \\
& \textbf{\name} & \bf 3.62 & 3.38 & \bf 3.41 & \bf 3.71  & \bf 3.89 & \bf 3.41 & \bf 3.41 & 3.41 \\

\hline


\end{tabular}}
%\vspace{0.1cm}
\caption{Scores for human evaluated metrics - Informativeness (INF), Relevance (REL), Coherence (COH), Fluency (FLU) over text based extractive systems (KLSumm and TextRank), abstractive systems (PG and CopyTransformer), video based abstractive systems (Action features with RNN) and multimodel systems (FMT Encoder Decoder, MulT Language Model and \name\ ) on How2 and AVIATE datasets.}
\label{tab:human}
%\vspace{-6mm}
\end{table*}}

\newcommand{\fourthtable}{% no arguments
\begin{table}[hbtp]
\centering

\setlength{\extrarowheight}{0.8pt}

\resizebox{0.7\textwidth}{!}{

\begin{tabular}{c|c|c|c|c|c|c}

& \multicolumn{3}{c|}{\bf How2} & \multicolumn{3}{c}{\bf AVIATE} \\\cline{2-7}
& \bf R-1 & \bf  R-2 & \bf R-L & \bf R-1 & \bf  R-2 & \bf R-L \\
\hline

\bf How2 & 56.89 & 26.93 & 56.80 & 21.35 & 4.88 & 23.11 \\
\hline 
\bf How2 with ASR & 54.19 & 24.07 & 52.11 & 22.77 & 5.98 & 24.07
 \\
\hline
\bf AVIATE & 52.68 & 21.33 & 49.9 & 37.13 & 11.04 & 31.47 \\

\hline

\end{tabular}}
%\vspace{0.1cm}
\caption{Transferability of the proposed \name\  model on the two available multimodal abstractive text summarization datasets - How2 and AVIATE. The network is trained on the dataset in each row, and is tested on the dataset shown in each
column. The second row indicates the performance of \name\ on the How2 videos whose transcripts are generated from ASR.}
\label{tab:transferability}
%\vspace{-8mm}
\end{table} }



\newcommand{\fifthtable}{% no arguments

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\centering

\setlength{\extrarowheight}{0.1pt}

\resizebox{0.8\columnwidth}{!}{


\begin{tabular}{c|l|l}
\multicolumn{1}{l|}{Task}     & Hyperparameter        & Value    \\ \hline
\multirow{5}{*}{Pre-training} & Vocab Size            & 50000    \\
                              & Text Input Embedding  & 768      \\
                              & Learning Rate         & 0.01     \\
                              & Optimizer             & Adam     \\
                              & Betas                 & 0.9,0.98 \\ \hline
\multirow{9}{*}{Fine-tune}    & Video input Embedding & 2048     \\
                              & Audio input Embedding & 40       \\
                              & ASR, OCR input Embedding   & 768      \\
                              & Optimizer             & Adam     \\
                              & Betas                 & 0.9,0.98 \\
                              & Convolution Dimension & 3        \\
                              & Epochs                & 300      \\
                              & Dropout               & 0.2      \\ 
                              & Text Embeddings       & bert-base-cased \\ \hline
\end{tabular}}
%\vspace{0.1cm}
\caption{Hyperparameters used in \name.}
\label{tab:hyper}
%\vspace{-10mm}
\end{table}}


\newcommand{\sixthtable}{% no arguments

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbtp]
\begin{tabular}{l|l}

\setlength{\extrarowheight}{0.8pt}

\resizebox{0.8\columnwidth}{!}{

\hline
Set &
  Tokens \\ \hline
Reference Summary &
  the, of, and, a, to, in, that, on, for, We, is, we, with, model, this, as, by, are, from, our, an, which, In, models, show, language, neural, can, propose \\
Model Summary &
  the, of, and, a, to, on, we, that, for, with, model, we, propose, this, in, neural, by, is, it, has, are, linguistic, novel, proposed, language, show, machine \\ \hline
\end{tabular}}
\end{table}}



\newcommand{\seventhtable}{% no arguments
\begin{table}[hbtp]
\centering

\setlength{\extrarowheight}{0.8pt}

\resizebox{0.7\textwidth}{!}{

\begin{tabular}{c|c|c|c|c|c|c}

& \multicolumn{3}{c|}{\bf How2} & \multicolumn{3}{c}{\bf AVIATE} \\\cline{2-7}
& \bf R-1 & \bf  R-2 & \bf R-L & \bf R-1 & \bf  R-2 & \bf R-L \\
\hline

\bf How2 & 56.89 & 26.93 & 56.80 & 21.35 & 4.88 & 23.11 \\
\hline
\bf AVIATE & 52.68 & 21.33 & 49.9 & 37.13 & 11.04 & 31.47 \\

\hline

\end{tabular}}
%\vspace{0.1cm}
\caption{{Transferability of the proposed \name\  model on the two available multimodal abstractive text summarization datasets - How2 and AVIATE. The network is trained on the dataset in each row, and is tested on the dataset shown in each
column.}}
\label{tab:transferability}
%\vspace{-8mm}
\end{table} }

==> table_figures/table_sample_summary.tex <==
\begin{table*}[hbtp]
  \centering
%   \renewcommand{\thetable}{A1}
  \setlength{\extrarowheight}{12pt}
  \scalebox{0.5}{
  \begin{tabular}{p{2.7cm} | c | p{15.5cm}}
    \toprule
    \bf Model & \bf R-L & \bf Output \\
    \hline
    \hline
    \midrule
    Ground-truth   & - & \small We study the problem of semi-supervised question answering—utilizing unlabeled text to boost the performance of question answering models. We propose a novel training framework, the Generative Domain-Adaptive Nets. In this framework, we train a generative model to generate questions based on the unlabeled text, and combine model-generated questions with human-generated questions for training question answering models. We develop novel domain adaptation algorithms, based on to learn richer context-aware model on the insight and the human-generated data distribution. Experiments show that our proposed framework obtains substantial improvement from unlabeled text. \\ [0.05cm]
    
    
    \name\ (ours) & 31.47 & \small We study \textcolor{red}{the problem of semi-supervised} concepts unlabeled text to boost the \textcolor{blue}{performance of without without models}. We propose a novel training framework, \textcolor{red}{the Generative Domain-Adaptive Nets. In this framework, we train} a database model and generate concepts based on procedure on how partitioning in the levels between t, \textcolor{red}{and combine model-generated} \textcolor{blue}{attention with} human-generated \textcolor{red}{types for training associations} directed-generation models. We develop novel algorithms, based on model, to understand \textcolor{blue}{the discrepancy between} the generated data results \textcolor{red}{ and the human-generated data distribution. Experiments show} model obtains improvement from text. \\  [0.05cm] 
    MultT LM  & 28.73 & \small In learn paper are neural paper, we propose a new model and the paper, we \textcolor{blue}{study demonstrated the character score} We \textcolor{red}{investigate the problem answering utilizing unlabeled text} to understand trained models. we train a understanding model to generate understanding based on the text, and \textcolor{red}{combine trained understanding with human generated} understanding to training data trained we \textcolor{blue}{assume like, on a public unsupervised Subsequently}, \textcolor{red}{prediction trained to learn richer context-aware model on the insight} In trained facilitates smaller annotations previously reported understanding understanding on approach and questions \textcolor{blue}{along five perform two then} performance The the semantic best dataset and the proposed \\ [0.05cm]
    MultT En-De & 27.2 & \small We present the problem of supervised new \textcolor{red}{utilizing text of} new new models. We propose a problem model review a new model In this paper, we propose a simple model Experimental results\textcolor{red}{ prove the standard model achieves} method to then the proposed among review model to also performance based on the \textcolor{blue}{proposed CoNLL-2012 dataset}. \textcolor{red}{In this we train a new model to generate a} model and combine model. \textcolor{blue}{of machine morphology into more prediction on the drawback of the system classes}. \textcolor{blue}{using error-correcting codes collection.} We evaluate \textcolor{blue}{investigation of NMT and induced Experiments errors. shed light affect vs. scores} on a word its dataset with the proposed based \\ [0.05cm]
    CopyTrans.  & 27.06 & \small We propose a novel method for novel method for state-of-the-art \textcolor{red}{question answering} we show that the  method achieves state-of-the-art performance on the state-of-the-art performance of the proposed method on the systems \textcolor{blue}{over sequential text tasks or as independent, parallel tasks.} \textcolor{red}{In this framework model generate text} trained \textcolor{blue}{benefits of the new semantic high a image} and at them as \\ [0.05cm]
    HA  & 26.12 & \small We propose the novel model has the paper, we \textcolor{red}{propose a generative model} In both learning can can the benchmark model To capable to \textcolor{blue}{also performance of existing the pipelined of the model-generated model}: distribution for the \textcolor{red}{human-generated data distribution}. Experiments show that our proposed framework to the consistency of the \textcolor{blue}{art data distribution and event feedforward network}. The an unsupervised dependency framework performance and the human data distruction . \\ [0.05cm]
    PG  & 23.81   & \small In this paper we consider the problem of learning a deep neural network, \textcolor{red}{we propose a novel neural network architecture} based on novel neural network architecture that is \textcolor{blue}{trained end-to-end trainable convolutional neural network (CNN) architecture} \textcolor{red}{is able to train} \textcolor{blue}{a convolutional neural network architecture} that is capable of achieving state-of-the-art performance compared to state-of-the-art performance on three benchmark datasets. \\ [0.2cm]
   PG-MMR & 22.63 & \small We propose a novel method \textcolor{blue}{for object detection based on a novel object detection method} that uses a \textcolor{blue}{novel model based on the posterior distribution of the posterior distribution} over the parameters of the \textcolor{blue}{number of claims} and We show that  models can be used as well as compared to In this paper, we study the a algorithm that the proposed method can  outperforms the state-of-the-art methods on a large number of \\  [0.05cm]
    \bottomrule
    \hline
\end{tabular}}
  \caption{Comparison of ground-truth summary and outputs of $7$ different unimodal and multimodel abstractive text summarization systems - \name, MultT LM, MultT Encoder-Decoder, CopyTransformer, multimodal hierarchical attention (HA), Pointer Generator (PG) and Pointer Generator with MMR (PG-MMR) - arranged in the order of best to worst ROUGE-L scores in this table. \textcolor{red}{Red} highlighted text indicates a \textcolor{red}{positive} correlation of context w.r.t. ground-truth summary while \textcolor{blue}{blue} color represents a \textcolor{blue}{negative} correlation with ground-truth summary.}
  \label{tab:output_examples}
\end{table*}
